CurveFusion: Reconstructing Thin Structures from RGBD Sequences

We introduce CurveFusion, the first approach for high quality scanning of thin structures at interactive rates using a handheld RGBD camera. Thin filament-like structures are mathematically just 1D curves embedded in R^3, and integration-based reconstruction works best when depth sequences (from the thin structure parts) are fused using the object's (unknown) curve skeleton. Thus, using the complementary but noisy color and depth channels, CurveFusion first automatically identifies point samples on potential thin structures and groups them into bundles, each being a group of a fixed number of aligned consecutive frames. Then, the algorithm extracts per-bundle skeleton curves using L1 axes, and aligns and iteratively merges the L1 segments from all the bundles to form the final complete curve skeleton. Thus, unlike previous methods, reconstruction happens via integration along a data-dependent fusion primitive, i.e., the extracted curve skeleton. We extensively evaluate CurveFusion on a range of challenging examples, different scanner and calibration settings, and present high fidelity thin structure reconstructions previously just not possible from raw RGBD sequences.

==> introduction.tex <==
%!TEX root = main.tex
\section{Introduction}


The last few years have seen significant research progress in the context of scanning of large-scale indoor environments. With easy access to depth cameras producing real-time feed of RGBD sequences, the most successful approach has been to align and integrate many such low-quality input frames, and extract a {\em fused} surface.  Well known examples include KinectFusion~\cite{Newcombe:2011}, BundleFusion~\cite{Dai:2017}, etc. 

The above family of methods implicitly assumes that the scanned environments to consist of volumetric objects with closed boundary surfaces. Hence, multiple depth scans, once aligned, can be effectively integrated using a (truncated) signed distance field representation discretized on a voxel grid, and a final surface extracted using marching cube (or its variants). 
%
\if0
\duygu{Do we need the following sentence since this is not exactly the same problem as us?}Only very recently the approach has been extracted to handle thin surfaces~\cite{tubiblio89320}. 
\fi


Such volumetric fusion approaches simply fail to capture objects or object parts primarily consisting of thin structures. Figure~\ref{xx} shows a typical result of a scanning session. The signal from the thin parts are either noisy, or even worse, completely missed in the original raw depth maps. Hence, thin structures get lost in the fused output. %
Generally, capturing thin structures by `fusing' several RGBD frames is challenging on multiple counts: 
(i)~depth channel returns unreliable signal -- parts of thin structures are regularly missed, and there is no  connectivity information among the few detected points; 
(ii)~RGB provides noisy information at best since it is very difficult to  differentiate between curve edges and texture/background edges; and
(iii)~fusion primitive is unknown to start with -- both connectivity and geometry, while using a predetermined fusion data structure (e.g., a voxel grid) is unsuited. 
% 
Essentially, both data channels (i.e., RGB and depth) are noisy. 


Given noisy RGBD measurements, simple attempts to recover 3D thin structures fail. For example, as shown in Figure~\ref{fig:RGBD_motivation} 
attempts to `lift' 2D curves from RGB images to 3D thin structures using depth images fails on two counts: first, detecting correct curve edges is difficult due to ambiguity with background edges; and second, even if one can detect corresponding curve edges, giving them depth is challenging due to unreliable or completely missing depth information.  

\begin{figure}[t!]
    \centering
    %\includegraphics{}
    \vspace{1.5in}
    \caption{show depth + image inputs; lifting fails; show fusion fails. shows baseline methods}
    \label{fig:RGBD_motivation}
\end{figure}



We take a different avenue --- 
starting from RGBD frames, we propose a reconstruction approach for thin structures that uses a fusion-primitive that is data-dependent, rather than being pre-authored. Specifically, 
our method discovers underlying 3D skeletons that characterize the scanned thin structures by jointly extracting information from both image and depth channels. Algorithmically, we consolidate burst of raw depth frames into mutually-aligned {\em bundles} and identify groups of consolidated points in each bundle coming from thin-structures using both image and depth information. We extract $L_1$ skeletons from such consolidated points. Given $L_1$ curve fragments extracted from different bundles of frames, we propose a novel curve consolidation algorithm to obtain a final 3D skeleton curve. In this step, we explicitly detect {\em junctions} (i.e., where three or more curve segments meet in 3D) and retain them through the consolidation stage. The extracted 3D skeleton is then used to recover back the final 3D surface of the scanned thin structures. Figure~\ref{fig:teaser} shows example results. 





\niloy{TODO Evaluation, results, ..} 
In summary,  we (i)~develop a first method to perform high-quality 3D curve reconstruction from raw RGBD data; (ii)~propose a data-dependent fusion approach that first discovers a suitable skeleton directly from the data and then uses it for reconstruction; and (iii)~present capture results of thin structures previously not possible from raw RGBD sequences. 
